Significant challenges for astrophysical inference with next-generation gravitational-wave observatories

The next generation of gravitational-wave observatories will achieve unprecedented strain sensitivities with an expanded observing band. They will detect ${\cal O}(10^5)$ binary neutron star (BNS) mergers every year, the loudest of which will be in the band for $\approx 90$ minutes with signal-to-noise ratios $\approx 1500$. Current techniques will not be able to determine the astrophysical parameters of the loudest of next-gen BNS signals. We show that subtleties arising from the rotation of the Earth and the free-spectral range of gravitational-wave interferometers dramatically increases the complexity of next-gen BNS signals compared to the one-minute signals seen by LIGO--Virgo. Various compression methods currently relied upon to speed up the most expensive BNS calculations -- reduced-order quadrature, multi-banding, and relative binning -- will no longer be effective. We carry out reduced-order inference on a simulated next-gen BNS signal taking into account the Earth's rotation and the observatories' free-spectral range. We show that standard data compression techniques become impractical, and the full problem becomes computationally infeasible, when we include data below $\approx 16$Hz -- a part of the observing band that is critical for precise sky localisation. We discuss potential paths towards solving this complex problem.

==> old/old_formalism_with_comments.tex <==
In this section we describe the construction of a reduced order model for a binary neutron star waveform. 
{\color{red}[Eric: add text describing the basic idea of ROM construction.]}




\subsection{Construction Techniques}
{\color{red}[The next two sections are lacking in context, details, and explanation. \textbf{This needs to be written so that someone like Nir can understand every paragraph.} The slides that you presented at our group meeting are the right level. Let's look at just the first sentence...}
The training set waveforms used to construct the reduced order models are evaluated over adaptively sampled frequency domains as outlined in \cite{Smith_2016}. 
{\color{red}[What training set waveforms? Take a big step back and set the stage so that we are not stepping directly onto $\unit[100]{km \, hr^{-1}}$ train! And what is the adaptively sampled frequency domains outlined in Smith? Why are we doing that? (The next sentence explains that this reduces the memory requirements, but it's too late: your reader is already confused. Explain what the memory issue is / how it arises. Then explain how Smith solves it.]}

{\color{red}Eric: these two subsections should have bullet lists breaking down the ROM building into easy-to-understand steps. There should be some equations to explain how things work.}
This technique reduces the memory requirements of a faithful training set by splitting the frequency domain into bands $b$ in powers of two and resampling with an adaptive resolution $\Delta f^{(b)}$ based on the time spent in each band. This reduces the cost of the training set by $\mathcal{O}(10^2)$ and enables fast construction of faithful bases.

The post-Newtonian expansion of the time to merger $t(f)$ is utilised to adaptively sample the bands, and this approximation breaks down near the inner-most stable circular orbit. Therefore, we extend upon the method outlined in \cite{Smith_2016} by limiting the maximum frequency resolution to $\Delta f^{(b)} = 1$ to mitigate under-sampling high-frequency bands. This has negligible effects on the compression of the training set.

To preserve faithfulness, the basis is up-sampled to the uniform frequency domain by performing the reduced basis algorithm over faithful waveforms evaluated at the greedily selected parameters $\{\lambda_i\}_i^{N_L}$ identified from the down-sampled training set. Rerunning the reduced basis algorithm to build a faithful basis tracks the projection errors to validate the adaptive sampling procedure. 

We also employ an iterative enrichment scheme to increase the effective size of the training set. By building arbitrarily many supplementary training sets, we can repeat the reduced basis greedy algorithm on each training set for a larger effective training set volume. This technique is motivated by memory constraints for constructing the basis, often requiring over terabytes of memory and several hundred CPUs.

\subsection{Populating the Training Set}
Constructing reduced order models for the detector response in Eq.~\ref{eq:detectorresponse} requires including the right ascension RA, declination DEC, time of coalescence $t_c$, and polarisation angle $\psi$. These parameters are ignored in previous studies and significantly increase the dimensionality of the training set. Therefore, a sophisticated strategy for populating the training set is imperative to reducing the number of reduced basis elements. 

We compose the training set of $N$ randomly chosen samples from the prior and $N$ samples taken from uniform grids in all parameters except chirp mass. Instead, we sample uniformly in $\mathcal{M}^{-5/3}$ as this describes the phase of the inspiral to leading order. Additionally, all boundary parameter samples are included in the training set. As the space of waveforms is in general slowly varying and smooth, much of the variance is in samples at the edges in parameter space. 

Unlike previous work \citep{Smith_2016, rory, morisakai_2020_froq}, we construct the reduced basis using the noise-weighted inner product in Eq.~\ref{eq:nwip}. Therefore, the greedy algorithm selects basis elements that are more informative with respect to the likelihood calculations in Eq.~\ref{eq:loglikelihood}, further decreasing the size of the basis.

Despite these construction techniques, the inclusion of the effects of Earth's rotation and the free spectral range cause the size of the basis to grow by many orders of magnitude. This presents a significant challenge for binary neutron star signals starting from $f_{\text{min}}=5$Hz where constructing a basis becomes computationally infeasible.


\section{Accuracy of Reduced Order Quadrature}\label{sec:likelihood_accuracy}
% Eric: I've deleted the intro text that was here. 

The evaluation of the log likelihood in Eq.~\ref{eq:loglikelihood} presents a major computational bottleneck for the parameter estimation of gravitational wave signals. This is because it involves evaluating the waveform over $L=\texttt{int}[T\cdot(f_{\max}-f_{\min}]$ frequency points. The empirical interpolant of the waveform $h$ in the frequency domain is defined as \citep{Barrault_2004}
\begin{align}
    \label{eq:ei}
    h^{\text{EI}}(f,\lambda) &= \sum_{j=1}^{N} h(F_j,\lambda)B_j(f).
\end{align}
{\color{red}[Eric: this should come earlier in our overview of how ROMs work.]}
Here, $B(f)$ is an interpolation matrix formed from the reduced basis $\{e_i\}_i^{N}$, and $h(F_j)$ is the waveform evaluated at frequency points from a set of greedily selected frequencies $\{F_i\}_i^{N}$ that minimises the error in the approximation. Furthermore, $N$ is the number of frequency nodes, and therefore the number of basis elements. 
{\color{red}Eric: this is impenetrable if we don't first explain the basic math of how this works.}

The empirical interpolant can be utilised to construct an efficient approximation to the log likelihood. We construct ROMs for $h$ annd $|h|^2$, referred to as the linear and quadratic ROMs, respectively. The quadratic basis is generally smaller than the linear basis as it does not need to capture the complex phase of the detector response, and therefore provides better likelihood compression. Substituting the empirical interpolant into Eq.~\ref{eq:loglikelihood}, we obtain the reduced order quadrature log likelihood
\begin{align}
    \label{eq:roq}
    \ln \mathcal{L} \propto &\sum_{j=1}^{N_L} h(F_j,\lambda) \omega_j -\frac{1}{2}\sum_{i=1}^{N_Q}|h(F_i,\lambda)|^2\psi_{i} - \frac{1}{2}\mathcal{Z}_n.
\end{align}
The number of basis elements, and therefore frequency nodes, of the linear model and quadratic model are given by $N_L$ and $N_Q$. Since the reduced order quadrature likelihood only needs to be evaluated at $N_L+N_Q$ frequency points, the compression of the log likelihood is in general
\begin{align}
    \label{eq:speedup}
    \frac{L}{N_L+N_Q} \gg 1.
\end{align}
For a typical binary neutron star signal in Cosmic Explorer ignoring the effects due to Earth's rotation and the free spectral range, the likelihood compression is $L/(N_L+N_Q)=\mathcal{O}(10^4)$. 

In Eq.~\ref{eq:roq}, $\omega_j$ and $\psi_{i}$ are integration weights that only need to be computed once offline. The weights are given by 
\begin{align}
    \label{eq:weights}
    w_j &= 4\Delta f\sum_{k=1}^{N_L} \frac{d^*(f_k)B_j(f_k)}{S_n(f_k)}, \\
    \psi_{i}&= 4\Delta f\sum_{k=1}^{N_Q}\frac{C_i(f_k)}{S_n(f_k)},
\end{align}
where $d(f_k)$ is the data and $S_n(f_k)$ is the power spectral density. 

The phase of the detector response in Eq.~\ref{eq:detectorresponse} is not included in our weight calculation as it is captured by our reduced order model, unlike those seen in, e.g., \cite{rory, Morisaki_2023}. This is necessary to include the time and frequency dependence of the phase due to the effects of Earth's rotation. Previous studies interpolate the weights over a fine grid in parameter space to accommodate the phase. Therefore, our ROQ rule is more lightweight and requires a cheaper offline cost.

We derive an approximate relation between the relative error in the log likelihood ratio $\Delta \ln \mathcal{L}/\ln \mathcal{L}$ and the maximum signal-to-noise ratio $\rho$ able to be studied by a reduced order quadrature rule, given by 
\begin{align}\label{eq:delta_ll_snr}
    \frac{\Delta \ln \mathcal{L}}{\ln \mathcal{L}} &\lesssim \frac{2}{\rho^2}.
\end{align}
The likelihood error is defined as $\Delta\ln\mathcal{L} = \ln\mathcal{L} - \ln\mathcal{L}_{\text{ROQ}}$ where $\ln\mathcal{L}$ is the standard likelihood and $\ln\mathcal{L}_{\text{ROQ}}$ is the ROQ likelihood. Details on the derivation are given in Appendix~\ref{sec:aprior}. 

{\color{red}[Eric: everything in this subsection up to this point can probably be moved into an earlier section thats explains the foundational concepts of ROMs. This is where we get into the bit about what you have done for this paper.]}

We construct reduced order models for the detector response described in Eq.~\ref{eq:detectorresponse}, which includes the full set of effects due to the free spectral range and Earth's rotation. 
{\color{red}[Eric: the subsequent sentence only makes sense if we have already had a discussion about how the size of the basis explodes when we include the FSR and the rotation of the Earth.]}
We limit the maximum basis size to be 100 gigabytes to enable construction of reduced order models and practically feasible data analysis. 
The models are built with minimum frequencies $f_{\text{min}}$ in the range of $[22, 30]$Hz and to a maximum frequency of $2048$Hz. 
We build the ROM over the full parameter ranges for all parameters except the dimensionless spin magnitudes $a_{1,2}$ which we limit to $a_{1,2}\leq 0.05$, and the chirp mass $\mathcal{M}_c$. 

==> old/rom_er_fsr.tex <==

\subsection{Effects Due to Earth's Motion and The Free Spectral Range}\label{sec:er_fsr}
The minimum resolvable frequency of gravitational wave detectors determines the maximum duration a signal can spend in band. Over the hours-long signals expected to be observed by next-generation detectors, the detector will move through space as Earth rotates. Furthermore, as the size of the detector approaches the wavelength of the incident wave, the signal evolves over the travel time of photons in the detector arms. The frequency at which this occurs is the free spectral range. The result of both of these effects is that the antenna response functions $F^{+/\times}$ and the phase $\psi$ become frequency-dependent.

To obtain an expression for the frequency domain signal, we introduce time-dependence into our antenna response factors by defining
\begin{align}
    \label{eq:td_sig}
    h(t_c+t+\tau(t)) &= F^{+}(t)h^{+}(t) + F^{\times}(t)h^{\times}(t).
\end{align}
In this case, the light travel time $\tau$ is time dependent as the spatial location of the detectors $\mathbf{r}$ and the vector along the direction of propagation $\mathbf{n}$ are time dependent. 

The time-dependent antenna response factors are given by \citep{Essick_2017}
\begin{align}\label{eq:fpc}
    F^{+/\times}(t) &= D_{ij}(t)\epsilon^{ij, +/\times}(t),
\end{align}
where $D_{ij}(t)$ is the detector tensor, which describes the response of the interferometer to an incident wave, and $\epsilon^{ij}$ is the polarisation tensor, defined in \cite{Anderson_2001}. It is clear that the antenna response is a projection effect that maps the strains in the wave-frame onto the detector. However, these tensors depend on the orientation and dynamics of the detector which changes as the Earth rotates and at the free spectral range. 

The free spectral range effects enter only into the detector tensor $D_{ij}(t)$, defined as 
\begin{align}
    D_{ij}(t) &= D(f,n_k(t)e^k_x)e^i_xe^j_x - D(f,n_le^l_y)e^i_ye^j_y.
\end{align}
Here, $e_i$ are the unit-vectors oriented parallel to the detector arms, and $D(f,n_e)$ is the fractional change in the travel time for a single arm where $n_e=n_pe^p$, and is defined as \cite{Essick_2017}
\begin{align} \label{eq:d_f_ne}
    D(f,n_e) &= \frac{e^{-\pi i f/f_{\text{FSR}}}}{2(1-n_e^2)}\big[\sinc(\frac{\pi f}{f_{\text{FSR}}}) -n_e^2\sinc(\frac{\pi n_e f}{f_{\text{FSR}}}) - \frac{in_ef_{\text{FSR}}}{f}(\cos(\frac{\pi f}{f_{\text{FSR}}}) -\cos(\frac{\pi n_e f}{f_{\text{FSR}}}))\big].
\end{align}
As the Earth rotates, the unit vectors $e_i$ that describe the orientation of the detector become time dependent. Therefore, $D(f,n_e)$ is both time and frequency dependent. 

A common approximation in the limit of small detector size is
\begin{align}\label{eq:approx_d_f_ne}
    \lim_{\frac{f}{f_{\text{FSR}}}\rightarrow 0} D(f, n_e) &= \frac{1}{2} - \frac{\pi i f L}{c}(1-\frac{n}{2}).
\end{align}
Whilst the limit of $f/f_{\text{FSR}}\rightarrow 0$ straightforwardly excludes the effects of the free spectral range, it also ignores effects due to the Earth's rotation by removing the dependence on $e_i$. 

Including the time-dependent unit vectors in the definition of $D(f,n_e)$ causes the size of the reduced order models built in Chapter~\ref{sec:building_roms} to explode. Previous work studying binary neutron star signals in Cosmic Explorer with reduced order modelling ignores this effect and utilises the approximate version of $D(f,n_e)$ given in Eq.~\ref{eq:approx_d_f_ne} \cite{rory}. In this work, I incorporate the complete effects due to the Earth's motion and the free spectral range by utilising the unapproximated detector response.

%The time dependent antenna response factors are given by \citep{jaranowski}
%\begin{align}
%    F^+(t) &= \sin \xi[a(t)\cos 2\psi + b(t)\sin 2\psi] \\
%    F^{\times}(t) &= \sin \xi[b(t)\sin 2\psi - a(t)\cos 2\psi].
%\end{align}
%The angle $\xi$ is the angle between detector arms, and $\psi$ is the polarization angle of the gravitational wave source. The factors $a(t)$ and $b(t)$ are given in Eq.~12 $-$ Eq.~13 of \cite{jaranowski}.

The overarching effect of Earth's rotation and the free spectral range on the signal manifests as multiple phase and amplitude modulations due to the variation of the antenna response factors with time, as well as a Doppler shift due to the relative motion between the source and the detector \citep{cornish}. This Doppler shift originates from the time dependence of the light crossing time $\tau(t)$.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{phase_jacob_vs_constant.pdf}
    \caption[Frequency dependent phase and antenna factors]{\textit{Top:} The plus and cross polarised antenna response factors in Eq.~\ref{eq:fpc}. \textit{Bottom:} The detector response phase in Eq.~\ref{eq:phase}. All quantities are evaluated using Cosmic Explorer, a fixed source location and polarisation angle, and illustrated as frequency-dependent (yellow, crimson) and frequency-independent (blue, green).}
    \label{fig:fp_phase_vs_constant}
\end{figure}

%\begin{figure}
%\centering
%\begin{subfigure}{1\textwidth}
%\centering
%  \includegraphics[width=0.9\textwidth]{fp_jacob_vs_constant.pdf}
%\end{subfigure}

%\begin{subfigure}{1\textwidth}
%\centering
%    \includegraphics[width=0.9\textwidth]{phase_jacob_vs_constant.pdf}
%\end{subfigure}
%\caption[Frequency dependent phase and antenna factors]{\textit{Top:} The plus polarised antenna response factor in Eq.~\ref{eq:fpc}. \textit{Bottom:} The detector response phase in Eq.~\ref{eq:phase}.
%Both quantities are evaluated using Cosmic Explorer, a fixed source location and polarisation angle, and illustrated as frequency-dependent (yellow) and frequency-independent (blue).}
%\label{fig:fp_phase_vs_constant}

%\end{figure}

To obtain a frequency domain expression, we Fourier transform Eq.~\ref{eq:td_sig} %obtained by Fourier transforming the multipole moments $h^{\ell m}(t)$:
\begin{align}
    \label{eq:fourier_transform}
    \tilde{h}(f) &= \int_{-\infty}^{\infty} h(t) e^{i2\pi ft} dt =  \int_{-\infty}^{\infty} A(t) e^{i(2\pi ft-\phi(t))} dt, %= \int_{-\infty}^{\infty} A^{\ell m}(t) e^{i(2\pi ft-m\phi(t))} dt.
\end{align}
where we have made use of the post-Newtonian approximation to decompose the waveform model into its amplitude $A(t)$ and phase $\phi(t)$. Then, we apply the stationary phase approximation, which is valid provided the amplitude of the time domain signal varies slowly with respect to the phase. Under this scenario, the Fourier transform can be simplified by expanding the integral around the point of stationary phase $t^*$, determined by setting the time derivative of the argument of the exponent in Eq.~\ref{eq:fourier_transform} to zero:
\begin{align}
    \label{eq:tstar}
    \frac{d\phi(t)}{dt}\Big|_{t=t^*} &= 2\pi f.
\end{align}
Then, the argument of the exponent can be expanded around $t^*$ in a Taylor series to give 
\begin{align}
    2\pi ft-\phi(t) &\approx 2\pi ft^*-\phi(t^*) - \frac{1}{2}\ddot{\phi}(t^*)(t-t^*)^2 + \dots,
\end{align}
where we ignore terms of higher order than $(t-t^*)^2$. Then, the integral in Eq.~\ref{eq:fourier_transform} is \citep{Cutler_1994}
\begin{align}
    \label{eq:multipole_f}
     \tilde{h}(f) &\approx A(t^*) e^{i(2\pi ft^*-\phi(t^*))}\int_{-\infty}^{\infty} e^{-i\frac{1}{2}\ddot{\phi}(t^*)(t-t^*)^2} dt.
\end{align}
Integrating over the Taylor expansion in phase and reintroducing the form of our time-domain expression in Eq.~\ref{eq:td_sig} gives the frequency-domain detector response
\begin{align}
    \label{eq:detectorresponse}
    \tilde{h}(f) &= [F^+(t^*)\tilde{h}^+(f) + F^{\times}(t^*)\tilde{h}^{\times}(f)] e^{i\psi(t^*)},
\end{align}
where we have defined the phase
\begin{align}
    \label{eq:phase}
    \psi(t^*) &= 2\pi f t^*-\phi(t^*)-\frac{\pi}{4}.
\end{align}
The stationary point $t^*$ can be defined in terms of frequency through the following relation of the orbital frequency and the energy $E(f)$ and flux $F(f)$ of the binary \citep{Santamaria_2010}
\begin{align}
    \frac{df}{dt} &= -\frac{F(f)}{dE(f)/df},
\end{align}
and is given to lowest order in the post-Newtonian expansion by (setting $G=c=1$) 
\begin{align}
    \label{eq:pnlow}
    t^*(f) &= t_c - \frac{5}{256}\mathcal{M}_c^{-5/3}(\pi f)^{-8/3}.
\end{align}
The quantity $t^*(f)$ is referred to as the time to merger. Here, $\mathcal{M}_c$ is the chirp mass, defined in terms of the component masses $m_{1,2}$ as 
\begin{align}
    \mathcal{M}_c &= \frac{(m_1m_2)^{3/5}}{(m_1+m_2)^{1/5}}.
\end{align}
Now that $t^*$ is defined in terms of frequency, we have a completely frequency dependent detector response. The derivation of Eq.~\ref{eq:detectorresponse} is given in more detail in Sec. 3.2 of \cite{Iacovelli_2022}. The complete set of parameters that describe the detector response in Eq.~\ref{eq:detectorresponse} under the waveform model \texttt{IMRPhenomPv2\_NRTidalv2} are listed in Table~\ref{tab:params}.

In Fig.~\ref{fig:fp_phase_vs_constant}, I illustrate the behaviour of the frequency dependent antenna factors $F^{+/\times}(t^*(f))$ and phase $\phi(t^*(f))$ for Cosmic Explorer compared to when these functions are considered as frequency independent. The frequency dependent antenna factors exhibit large sweeping changes at the high-frequency regime due to the inclusion of free spectral range effects. Both the frequency dependent antenna factors and phase exhibit complex behaviour in the low-frequency regime due to the Earth's motion. The complex evolution of these components of the detector response are clearly unable to effectively be captured by the frequency independent approximation used in current analysis of gravitational wave data, illustrated in dashed blue and green. 




\begin{table}
    \centering
    \begin{threeparttable}
    \caption[Table of parameter definitions]{Definition of parameters used throughout this work and their prior distributions. Subscripts $i=1,2$ refer to the primary and secondary components of the compact binary, respectively. The reference frequency used throughout this work to define certain parameters is $f_{\text{ref}}=40$Hz. The inclination angle $\iota$ depicted in Fig.~\ref{fig:sourceframe} can be reconstructed from $\theta_{JN}$ at $f_{\text{ref}}$ in post-processing. This table is adapted from \cite{isobel_2021}.} %The spin and precession parameters that parameterise the \texttt{IMRPhenomPv2\_NRTidalv2} waveform model are used directly to construct the reduced order models. However, the standard \texttt{Bilby} spins and spin angles are used in inference. }
    \begin{tabular}{c|p{10cm}|c|c}
        \hline
        \hline 
        Parameter & Description & Prior & Units \\
        \hline
        $\mathcal{M}_c$  & Detector frame chirp mass & Uniform & $M_{\odot}$  \\
        $q$ & Mass ratio $q\equiv m_2/m_1$ & Uniform & $-$ \\
        %$a_i^{\dagger}$ & Dimensionless spin magnitude of $i$-th component & Uniform & $-$ \\ 
        %$\theta_i^{\dagger}$ & Tilt angle of $i$-th component & Sine & rad. \\ 
        %$\phi_{12}^{\dagger}$ & Difference in angle between in-plane spins & Uniform & rad. \\ 
        %$\phi_{JL}^{\dagger}$ & Difference between total and orbital angular momentum angles & Uniform & rad. \\ 
        $\chi_i$ & Aligned spin of the $i$-th component & Uniform & $-$\\ 
        $\chi_p$ & Effective precession spin \cite{Hannam_2014} & Uniform & $-$ \\  
        $\alpha_0$ & Orientation of the orbital angular momentum at a reference frequency & Uniform & rad. \\ 
        $d_L$ & Luminosity distance to the source & Comoving & Mpc \\
        RA & Right ascension & Uniform & rad. \\
        DEC & Declination & Cosine & rad. \\ 
        $\theta_{JN}$ & Angle between total angular momentum and line of sight & Sine & rad. \\
        $\psi$ & Polarisation angle & Uniform & rad. \\ 
        $\phi_c$ & Phase at coalescence & Uniform & rad. \\ 
        $t_c$ & Time of coalescence & Uniform & sec. \\ 
        $\Lambda_i$ & Tidal deformability of the $i$-th component & Uniform & $-$ \\
        \hline
        \hline
    \end{tabular}
    %\begin{tablenotes}
    %  \small
    %  \item $^*$ Used only in ROM construction.
    %  \item $^{\dagger}$ Used only in inference.
    %\end{tablenotes}
    \label{tab:params}
    \end{threeparttable}
\end{table}

In the next Section, I describe reduced order modelling and building models of the detector response in Eq.~\ref{eq:detectorresponse}. Previous work ignores the complete set of effects on the detector response from the free spectral range and Earth's motion, as well as excluding the phase of the detector response from the reduced order model. Including these detector effects introduces frequency dependent phase terms that dramatically increase the size of the reduced order model, severely limiting the accuracy of the model and the acceleration of inference. 


\subsection{Reduced Order Modelling}
The parameter space for gravitational waveforms exhibit levels of redundancy that make such waveforms amenable to sparse representations \citep{Galley_2010}. A technique to construct a sparse representation for these models is reduced order modelling. Combining the reduced basis and empirical interpolation methods \citep{Barrault_2004} provides fast-to-evaluate surrogate models that can be arbitrarily accurate \citep{Field_2012}. Reduced order modelling is particularly useful in gravitational wave astronomy as it enables the construction of a reduced order quadrature (ROQ) likelihood, an approximate representation of the likelihood in Eq.~\ref{eq:likelihood}. Such an approximation is responsible for remarkable acceleration of parameter estimation \citep{speedup} as it reduces likelihood evaluations from being over the entire frequency domain, which can be up to $\mathcal{O}(10^{7})$ points, to over a few hundred judiciously chosen nodes. %However, in this work I show that the introduction of the effects due to Earth's rotation and the free spectral range in Eq.~\ref{eq:detectorresponse} causes reduced order modelling to become extremely limited in both the acceleration and accuracy of inference. 

\subsubsection{The Reduced Basis and Empirical Interpolant}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{linear_error.pdf}
    \caption[Reduced basis approximation error]{The maximum reduced basis approximation error onto a training set of 2 million binary neutron star merger signals. The signals are constructed  with a minimum frequency of $f_{\min}=15$Hz. The decay in the approximation error is exponential in the number of basis elements, as can be seen by the relation between the logarithm of the vertical axis and the horizontal axis. The tolerance  for the maximum approximation error was set to $\epsilon=10^{-16}$. At this error scale, numerical precision errors dominate and the mismatch between waveforms can become negative. This is why we observe a sharp drop at the $460$th basis element - it is computationally infeasible to make a basis that is any more accurate.}
    \label{fig:rb_error}
\end{figure}

The reduced basis method hierarchically constructs an orthonormal basis from a training set of waveforms that is a nearly optimal representation of the space of waveforms. Unlike other basis construction techniques such as principal component analysis (PCA) or proper orthogonal decomposition (POD), the reduced basis technique seeks to minimise the maximum projection error of the basis. This is crucial in setting confident upper-bounds on the maximum signal-to-noise ratio of signals that the reduced order models can approximate without introducing biases. The reduced basis algorithm iterates until the maximum projection error onto the basis of all training set waveforms is less than the user-defined tolerance. In Fig.~\ref{fig:rb_error}, I plot the maximum approximation error for a reduced basis as a function of the number of basis elements needed to approximate a training set of $2\times10^6$ binary neutron star waveforms starting from a minimum frequency of $f_{\min}=15$Hz detected with Cosmic Explorer. Only 460 basis elements are required to represent the millions of waveforms with a maximum approximation error less than $10^{-14}$, illustrating the sparse nature of the gravitational waveform parameter space. At the 460th basis element, the logarithm of the error drops sharply to negative infinity. This is because the tolerance I set on the maximum approximation error was $\epsilon=10^{-16}$, which is at the same scale as numerical precision errors. These numerical errors may render the mismatch in Eq.~\ref{eq:mismatch} negative, and hence it is not possible to achieve a more accurate basis without the use of higher precision floating point numbers. However, this would greatly increase the computational burden of constructing training sets.

The empirical interpolation method creates a weighted sum based on an interpolation matrix, which is constructed from combinations of the reduced basis elements. The weights correspond to evaluations of the true waveform model at a specific set of empirical nodes. The interpolant is built hierarchically by identifying the frequencies where it deviates most from the true waveform and then ensuring it matches the true waveform exactly at this frequency. The selected frequencies are the empirical interpolation nodes, with one unique node for each basis element. Consequently, the number of frequency nodes equals the number of basis elements, establishing an important relationship between the number of basis elements and the sparsity of the waveform model representation. In Fig.~\ref{fig:ei_nodes}, I illustrate in the top panel the amplitude of the empirical interpolant for a binary neutron star signal and overlay the empirical nodes. In the bottom panel, I plot a histogram of the number of empirical nodes as a function of frequency. Clusters of empirical nodes signify the regions of the signal that change most rapidly in parameter space, and these form at low and high frequencies due to the additional parameter dependence introduced by the effects of Earth's rotation and the free spectral range. For a more mathematical description of the reduced basis and empirical interpolation algorithms, I refer the reader to Appendix~\ref{appendix:rb_ei}. 


\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{fnodes.pdf}
    \caption[Empirical interpolant and frequency nodes]{\textit{Top:} The magnitude of the empirical interpolant in blue as a function of log frequency. The empirical interpolation nodes are  overlayed in orange. \textit{Bottom:} The distribution of empirical interpolation nodes as a function of frequency. The majority of nodes collect in the low-frequency regime. This is expected due to the complex behaviour at low frequencies introduced by the effects of Earth's rotation and the free spectral range.}
    \label{fig:ei_nodes}
\end{figure}

\subsubsection{The Reduced Order Quadrature Likelihood and Selecting a Model}
Armed with an extremely accurate and sparse representation of our waveform $h$, we can form a compressed version of the likelihood in Eq.~\ref{eq:likelihood}, referred to as a reduced order quadrature likelihood. The standard likelihood is evaluated over the uniform frequency domain, which has $N$ points where $N$ is defined as
\begin{align}
    N &= T\cdot (f_{\max} - f_{\min}),
\end{align}
where $T$ is the signal duration  and $f_{\max}$ is the maximum resolvable frequency, which I set to $f_{\max}=2048$Hz. The empirical interpolant replaces the uniform frequency dependence of the waveform with the sparse set of empirical nodes. By using the empirical interpolant instead of the waveform model in the likelihood, we only have to evaluate the likelihood over the empirical frequency nodes. This process involves an offline cost of building a set of likelihood weights, but this is computationally negligible. The log likelihood in Eq.~\ref{eq:loglikelihood} is composed of two inner products, with the signal appearing linearly in the first product and quadratically in the second. In this work, I construct a reduced order model for the waveform $h$ and its squared absolute value $|h|^2$, i.e. a separate model for each inner product. However, other studies use the linear model for both inner products. To justify my choice of model construction, I outline the speedup obtained by the reduced order quadrature likelihood with and without separate models for the inner products.

The number of basis elements, and therefore frequency nodes, of the linear model and quadratic model are given by $N_L$ and $N_Q$. Since the reduced order quadrature likelihood only needs to be evaluated at $N_L+N_Q$ frequency points where $N_L+N_Q\ll N$, the compression of the log likelihood is given by
\begin{align}
    \label{eq:speedup}
    \frac{N}{N_L+N_Q} \gg 1.
\end{align}
In general, the quadratic basis requires fewer elements than the linear basis as it does not need to capture the complex phase of the detector response. Therefore, $N_Q \leq N_L$ and 
\begin{align}
    \frac{N}{N_L+N_Q} \geq \frac{N}{2N_L}.
\end{align}
So, we get a better likelihood compression when using a quadratic basis to approximate $\langle h, h\rangle$ instead of using the linear basis. For a typical binary neutron star signal in Cosmic Explorer, the likelihood compression is $N/(N_L+N_Q)=\mathcal{O}(10^4)$.

%Earth's rotation introduces an explicit time dependence in the phase of the detector response in Eq.~\ref{eq:detectorresponse}. This time dependence is ignored in previous studies (e.g., \cite{rory, Morisaki_2023}) and the phase is absorbed into the likelihood weight construction. As the phase is nonetheless parameter dependent, the reduced order quadrature integration weights are interpolated over a fine grid in parameter space. This requires a significantly more intensive pre-processing step, but reduces the overall size of the reduced basis by ignoring the complex morphology of the phase. However, as the phase depends non-linearly on time when including the effects of Earth's rotation this technique is no longer valid for our study. 

Previous studies (e.g., \cite{rory, Morisaki_2023}) construct reduced order models only for the plus and cross polarised gravitational waveforms, $h^{+/\times}$, to approximate the phase-independent detector response. This relies on the important caveat that a basis constructed for a model $h$ can accurately approximate amplitude modulations to this model provided the amplitude modulation is in the span of the basis. In this case, the amplitude modulation is the parameter dependent antenna pattern functions $F^{+/\times}$. However, the basis fails to approximate the modulations introduced by the antenna pattern functions when properly accounting for the combined effects due to Earth's rotation and the free spectral range due to their complex behaviour as demonstrated in Fig.~\ref{fig:fp_phase_vs_constant}.

Therefore, I construct reduced order models for the complete detector response in Eq.~\ref{eq:detectorresponse}. This provides a cleaner online/offline decomposition and shortens the pre-processing required to perform inference using reduced order models. Whilst it has been suggested to construct reduced order models for individual components of the response, I refer the reader to Appendix~\ref{appendix:roq_choice} for a demonstration that such a choice is computationally inefficient.

\subsubsection{Earth's Rotation and the Free Spectral Range Break Reduced Order modelling}

Including the effects due to Earth's rotation and the free spectral range as described in Sec.~\ref{sec:er_fsr} causes an extreme increase in the size of the reduced basis. This is particularly prohibitive for the signals expected to be observed with Cosmic Explorer, so much so that construction is often impossible and the accuracy and likelihood acceleration promised by reduced order modelling is severely limited. Whilst previous work strives to demonstrate that reduced order models can provide fast and accurate inference for next-generation detectors (e.g., \cite{rory}), they fail to properly include the effects due to the free spectral range and the Earth's rotation. 

The culprit of the increase in basis size is the multiple frequency-dependent phase terms that are introduced into the detector response  when including the effects due to the Earth's rotation and the free spectral range. Most of these phase terms arise from the detector tensor amplitude described in Eq.~\ref{eq:d_f_ne}, but are also introduced through the polarisation tensor in Eq.~\ref{eq:fpc} as well as the phase of the detector response in Eq.~\ref{eq:detectorresponse}. As the reduced basis selects waveforms that differ based on their structure - not amplitude - quickly varying frequency dependent phase terms causes an enormous increase in the complexity of the allowed waveform structure. This requires excessive basis elements to properly capture, and hence an extremely large reduced basis. The selection of basis elements based on difference in phase is illustrated in Fig.~\ref{fig:basiselements}, where I plot the first 3 normalised basis elements of a reduced basis constructed for the same training set of 2 million binary neutron star waveforms starting from $f_{\min}=15$Hz in Cosmic Explorer as in Fig.~\ref{fig:rb_error}. Each basis element has a unique phase structure with respect to the other basis elements. I constrain the width of the frequency domain over which the basis elements are plotted to $\Delta f = 10^{-2}$ due to their rapid evolution.

%The reduced basis algorithm selects waveforms based on how different their structure is in comparison to other basis elements. The waveforms that compose the reduced basis are orthonormalised, and so constant amplitude changes are irrelevant to selecting waveforms. So, the primary source of changing structure in waveforms is changes in phase. Therefore, the many time dependent phase terms introduced to the detector response due to the Earth's rotation and the free spectral range introduce complex, quickly varying behaviour of the waveform over parameter space. 

%Whilst certain parameters directly influence the phase of the incident waveform, the phase is generally slowly varying as a function of the parameters and can be easily captured by the reduced basis. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{basis_elements.pdf}
    \caption[Elements of the reduced basis]{The first 3 normalised basis elements of a reduced order model constructed for 2 million binary neutron star waveforms starting from $f_{\min}=15$Hz in Cosmic Explorer. Each basis element is out of phase, illustrating how the phase structure can determine the selection of basis elements.}
    \label{fig:basiselements}
\end{figure}

%\textcolor{red}{INTRODUCE REDUCED ORDER modelling SIMPLY, IN SIMPLE LANGUAGE.}
%Introduce ROMs, describe them generally, and then state that we demonstrate that the inclusion of the full set of effects (FSR, earths rotation) causes ROM to explode. Make sure to mention that what we call a ROM is the empirical interpolant. Caused by inclusion of: detector response phase (which is time/frequency dependent under SPA), as the earth geocenter motion lag time becomes time dependent, and time dependent detector tensor (include FSR effects then also get low-frequency effects). Say this can be understood from Essick+ as the vector product $n_e$ changes as the vector $e$ changes as Earth rotates. Takeaway: ROMs are built based on shape of signal. Introducing these two phase shifts causes a huge paramater space of very different looking signals, causing the ROM to increase by 20 for 5Hz BNS. Then state that using various constraints we can recover this factor of 20 in compression and make/use the ROMs to properly analyse a 3G BNS signal.

In order to develop the reduced order models and perform the studies done in this work, I made significant contributions to the generalised reduced order modelling package \texttt{Rombus}. One of the most notable contributions was parallelising the construction of reduced order models. A parallelised reduced basis algorithm is vital for constructing reduced order models for signals that last longer than $T=1$ second. This is particularly relevant for next-generation detectors, where signals are expected to last for hours. Furthermore, I developed a number of gravitational wave specific techniques to improve the accuracy and efficiency of the reduced order model, as well as the reduced basis construction. Some of these methods are outlined in Chapter~\ref{sec:building_roms}. Finally, I have constructed a reduced order modelling inference pipeline to make the construction and use of reduced order models for fast and accurate gravitational wave inference available to everybody. For more extensive details on \texttt{Rombus} and my contributions, as well as the pipeline, I refer the reader to Appendix~\ref{appendix:rombus}.


Reduced order modelling is so far the only technique shown to reduce analysis times from years to hours with extreme precision in next-generation detectors \cite{rory}. However, previous work neglects the effects due to the free spectral range and relies on erroneous accuracy metrics. Other attempts at studying binary neutron star signals in Cosmic Explorer (e.g. \cite{baral}) use waveform approximants that are inaccurate at the signal-to-noise ratios studied, fix the spin parameters, and use a likelihood acceleration technique that does not provide reliable upper bounds on the allowed signal-to-noise ratio without introducing biases. In this work, I show that including the effects due to Earth's rotation and the free spectral range cause the size of the reduced basis to increase by many orders of magnitude. This severely limits the accuracy and acceleration of inference. As a result, there is currently no technique to reliably study many of the signals expected to be observed in next-generation detectors. However, I demonstrate for the first time accurate inference on a low signal-to-noise ratio signal in Cosmic Explorer including the effects of Earth's rotation and the free spectral range. Using reduced order modelling and the prescription laid out in this work, I reduce the inference time from 2 years to within an hour.

==> old/roq.tex <==
\textcolor{red}{This whole section could probably go into the appendix?}

The evaluation of the log likelihood in Eq.~\ref{eq:loglikelihood} presents a major computational bottleneck for the parameter estimation of gravitational wave signals. This is because it involves evaluating the waveform, which despite significant advances in waveform approximants remains slow for long and complex signals. In this Section, I introduce a reduced order quadrature likelihood expression by combining the empirical interpolant with the standard likelihood.

%Furthermore, I derive an approximate accuracy metric that relates the approximation error of the reduced order quadrature likelihood to the maximum signal to noise ratio that can be studied without introducing bias. As the accuracy of the reduced order model dictates the accuracy of the reduced order quadrature likelihood, this metric is useful in determining the required accuracy of a given reduced order model.




The empirical interpolant of the waveform $h$ in the frequency domain is defined as \citep{Barrault_2004}
\begin{align}
    \label{eq:ei}
    h^{\text{EI}}(f,\lambda) &= \sum_{j=1}^{N} h(F_j,\lambda)B_j(f).
\end{align}
Here, $B(f)$ is an interpolation matrix formed from the reduced basis $\{e_i\}_i^{N}$, and $h(F_j)$ is the waveform evaluated at frequency points from a set of greedily selected frequencies $\{F_i\}_i^{N}$ that minimises the error in the approximation. Furthermore, $N$ is the number of frequency nodes, and therefore the number of basis elements. 

The empirical interpolant can be utilised to construct an efficient approximation to the log likelihood. Substituting the empirical interpolant into Eq.~\ref{eq:loglikelihood}, we obtain the reduced order quadrature log likelihood
\begin{align}
    \label{eq:roq}
    \ln \mathcal{L} \propto &\sum_{j=1}^{N_L} h(F_j,\lambda) \omega_j -\frac{1}{2}\sum_{i=1}^{N_Q}|h(F_i,\lambda)|^2\psi_{i} - \frac{1}{2}\mathcal{Z}_n.
\end{align}
Here, $\omega_j$ and $\psi_{i}$ are integration weights that only need to be computed once offline. The weights are given by 
\begin{align}
    \label{eq:weights}
    w_j &= 4\Delta f\sum_{k=1}^{N_L} \frac{d^*(f_k)B_j(f_k)}{S_n(f_k)}, \\
    \psi_{i}&= 4\Delta f\sum_{k=1}^{N_Q}\frac{C_i(f_k)}{S_n(f_k)},
\end{align}
where $d(f_k)$ is the data and $S_n(f_k)$ is the power spectral density. The phase of the detector response in Eq.~\ref{eq:detectorresponse} is not included in our weight calculation as it is captured by our reduced order model, unlike those seen in, e.g., \cite{rory, Morisaki_2023}. This is necessary to include the time and frequency dependence of the phase due to the effects of Earth's rotation. These previous studies absorb the phase into the likelihood weight construction, but as the phase is parameter dependent the reduced order quadrature integration weights are interpolated over a fine grid in parameter space. By including the phase in the reduced order model construction, I massively reduces the offline computational cost of the weight calculation as the weights are no longer parameter dependent.
